The primordial binary population in the association Sco OB2

Observations over the last decade have indicated that a large fraction of the stars are part of a binary or multiple system. For our understanding of star formation it is therefore of crucial importance to characterise the outcome of the star forming process in terms of binary parameters. This thesis describes the recovery of the primordial binary population in the nearby OB association Sco OB2. The current binary population in Sco OB2 is first recovered using two adaptive optics surveys (ADONIS, NAOS-CONICA), a literature study, and a detailed analysis of the selection effects of visual, spectroscopic, and astrometric binary surveys. Our results indicate a binary fraction close to 100%. The mass ratio distribution (among A/B primaries) has the form f(q) = q^-0.4, while random pairing is excluded. The semi-major axis distribution has the form f(log a) = constant. Due to its youth and low stellar density, the current binary population of Sco OB2 is very similar to its primordial binary population. Our study further indicates a small brown dwarf companion frequency and a small substellar-to-stellar companion frequency among A and B type stars. These properties, often referred to as the brown dwarf desert, are a natural result of the mass ratio distribution in Sco OB2. The embryo ejection scenario is not necessary to explain observations. The brown dwarf desert may be ascribed to an excess of planetary companions, rather than by a lack of brown dwarf companions.

==> adonis_paper/table_all_edited.tex <==
HIP50520 &  &  & 6.23 & A1V &  &  & p & LCC &  \\
 &  &  & 6.39 &  & 2.51 & 313.3 & c &  &  \\
\hline
HIP52357 &  &  & 7.64 & A3IV &  &  & p & LCC &  \\
 &  &  & 7.65 &  & 0.53 & 73.0 & c &  &  \\
 &  &  & 11.45 &  & 10.04 & 72.7 & nc &  &  \\
\hline
HIP53524 &  &  & 6.76 & A8III &  &  & p & LCC &  \\
 &  &  & 12.67 &  & 4.87 & 316.9 & b &  &  \\
\hline
HIP53701 & 6.30 & 6.37 & 6.48 & B8IV &  &  & p & LCC &  \\
 & 9.05 & 8.76 & 8.86 &  & 3.88 & 75.8 & c &  &  \\
 & 13.06 & 12.93 & 13.04 &  & 6.57 & 120.1 & b &  &  \\
\hline
HIP54231 &  &  & 6.75 & A0V &  &  & p & LCC &  \\
\hline
HIP55188 &  &  & 7.43 & A2V &  &  & p & LCC &  \\
\hline
HIP55899 &  &  & 7.07 & A0V &  &  & p & LCC &  \\
\hline
HIP56354 &  &  & 5.78 & A9V &  &  & p & LCC &  \\
\hline
HIP56379 &  &  & 5.27 & B9Vne &  &  & p & LCC &  \\
\hline
HIP56963 &  &  & 7.46 & A3V &  &  & p & LCC &  \\
\hline
HIP56993 &  &  & 7.38 & A0V &  &  & p & LCC &  \\
 &  &  & 11.88 &  & 1.68 & 23.1 & nc &  &  \\
\hline
HIP57809 &  &  & 6.61 & A0V &  &  & p & LCC &  \\
\hline
HIP58416 &  &  & 7.03 & A7V &  &  & p & LCC &  \\
 &  &  & 8.66 &  & 0.58 & 166.1 & nc &  &  \\
\hline
HIP58452 &  &  & 6.51 & B8/B9V &  &  & p & LCC &  \\
\hline
HIP58465 &  &  & 6.32 & A2V &  &  & p & LCC &  \\
\hline
HIP58720 &  &  & 6.05 & B9V &  &  & p & LCC &  \\
\hline
HIP58859 &  &  & 6.52 & B9V &  &  & p & LCC &  \\
\hline
HIP59282 &  &  & 7.00 & A3V &  &  & p & LCC &  \\
\hline
HIP59397 &  &  & 7.01 & A2V &  &  & p & LCC &  \\
\hline
HIP59413 &  &  & 7.46 & A6V &  &  & p & LCC &  \\
 &  &  & 8.18 &  & 3.18 & 99.8 & c &  &  \\
 &  &  & 15.15 &  & 7.22 & 250.3 & b &  &  \\
\hline
HIP59502 &  &  & 6.80 & A2V &  &  & p & LCC &  \\
 &  &  & 11.28 &  & 2.94 & 26.4 & nc &  &  \\
 &  &  & 12.79 &  & 9.05 & 308.6 & b &  &  \\
\hline
HIP59898 &  &  & 5.99 & A0V &  &  & p & LCC &  \\
\hline
HIP60084 &  &  & 7.65 & A1V &  &  & p & LCC &  \\
 &  &  & 10.10 &  & 0.46 & 329.6 & nc &  &  \\
\hline
HIP60183 &  &  & 6.33 & B9V &  &  & p & LCC &  \\
\hline
HIP60561 &  &  & 6.59 & A0V &  &  & p & LCC &  \\
\hline
HIP60851 &  &  & 5.98 & A0Vn &  &  & p & LCC &  \\
 &  &  & 11.04 &  & 2.01 & 44.1 & nc &  &  \\
 &  &  & 11.66 &  & 6.92 & 181.1 & nc &  &  \\
\hline
HIP61257 &  &  & 6.60 & B9V &  &  & p & LCC &  \\
 &  &  & 12.43 &  & 5.54 & 324.3 & b &  &  \\
\hline
HIP61265 &  &  & 7.44 & A2V &  &  & p & LCC &  \\
 &  &  & 11.29 &  & 2.51 & 67.4 & nc &  &  \\
 &  &  & 14.70 &  & 3.43 & 168.6 & b &  &  \\
\hline
HIP61639 &  &  & 6.94 & A1/A2V &  &  & p & LCC &  \\
 &  &  & 7.06 &  & 1.87 & 182.4 & c &  &  \\
 &  &  & 14.36 &  & 4.21 & 220.6 & b &  &  \\
\hline
HIP61782 &  &  & 7.56 & A0V &  &  & p & LCC &  \\
\hline
HIP61796 &  &  & 6.37 & B8V &  &  & p & LCC &  \\
 &  &  & 11.79 &  & 9.89 & 109.0 & nc &  &  \\
 &  &  & 11.86 &  & 12.38 & 136.8 & nc &  &  \\
 &  &  & 13.35 &  & 4.17 & 305.8 & b &  &  \\
\hline
HIP62002 &  &  & 7.09 & A1V &  &  & p & LCC &  \\
 &  &  & 7.65 &  & 0.38 & 69.2 & c &  &  \\
 &  &  & 13.95 &  & 5.33 & 214.6 & b &  &  \\
\hline
HIP62026 &  &  & 6.49 & B9V &  &  & p & LCC &  \\
 &  &  & 7.46 &  & 0.22 & 12.5 & nc &  &  \\
\hline
HIP62058 &  &  & 6.17 & B9Vn &  &  & p & LCC &  \\
\hline
HIP62179 &  &  & 7.20 & A0IV/V &  &  & p & LCC &  \\
 &  &  & 7.57 &  & 0.23 & 282.7 & c &  &  \\
 &  &  & 14.03 &  & 12.21 & 131.3 & b &  &  \\
 &  &  & 14.60 &  & 4.47 & 255.8 & b &  &  \\
\hline
HIP63204 &  &  & 6.47 & A0p &  &  & p & LCC &  \\
 &  &  & 7.36 &  & 1.80 & 46.9 & nc &  &  \\
\hline
HIP63236 &  &  & 6.66 & A2IV/V &  &  & p & LCC &  \\
 &  &  & 12.91 &  & 7.56 & 118.4 & b &  &  \\
 &  &  & 12.85 &  & 11.97 & 316.5 & b &  &  \\
\hline
HIP63839 &  &  & 6.66 & A0V &  &  & p & LCC &  \\
 &  &  & 13.78 &  & 5.99 & 358.1 & b &  &  \\
 &  &  & 14.21 &  & 4.30 & 13.7 & b &  &  \\
 &  &  & 13.16 &  & 6.31 & 300.9 & b &  &  \\
\hline
HIP64320 &  &  & 6.22 & Ap &  &  & p & LCC &  \\
\hline
HIP64515 &  &  & 6.78 & B9V &  &  & p & LCC &  \\
 &  &  & 6.94 &  & 0.31 & 165.7 & c &  &  \\
\hline
HIP64892 &  &  & 6.82 & B9V &  &  & p & LCC &  \\
\hline
HIP64925 &  &  & 6.88 & A0V &  &  & p & LCC &  \\
\hline
HIP64933 &  &  & 6.29 & A0V &  &  & p & LCC &  \\
\hline
HIP65021 &  &  & 7.26 & B9V &  &  & p & LCC &  \\
\hline
HIP65089 &  &  & 7.37 & A7/A8V &  &  & p & LCC &  \\
\hline
HIP65178 &  &  & 6.71 & B9V &  &  & p & LCC &  \\
\hline
HIP65219 &  &  & 6.52 & A3/A4III/IV &  &  & p & LCC &  \\
\hline
HIP65394 &  &  & 7.25 & A1Vn... &  &  & p & LCC &  \\
\hline
HIP65426 &  &  & 6.78 & A2V &  &  & p & LCC &  \\
\hline
HIP65822 &  &  & 6.68 & A1V &  &  & p & LCC &  \\
 &  &  & 11.08 &  & 1.82 & 303.9 & nc &  &  \\
\hline
HIP65965 &  &  & 7.51 & B9V &  &  & p & LCC &  \\
 &  &  & 15.21 &  & 10.28 & 41.1 & b &  &  \\
\hline
HIP66068 &  &  & 7.04 & A1/A2V &  &  & p & LCC &  \\
\hline
HIP66447 &  &  & 7.16 & A3IV/V &  &  & p & UCL &  \\
\hline
HIP66454 &  &  & 6.33 & B8V &  &  & p & LCC &  \\
\hline
HIP66566 &  &  & 7.36 & A1V &  &  & p & LCC &  \\
\hline
HIP66651 &  &  & 7.35 & B9.5V &  &  & p & LCC &  \\
 &  &  & 15.36 &  & 7.58 & 173.3 & b &  &  \\
\hline
HIP66722 &  &  & 6.32 & A0V &  &  & p & UCL &  \\
\hline
HIP66908 &  &  & 6.86 & A4V &  &  & p & UCL &  \\
\hline
HIP67036 &  &  & 6.69 & A0p &  &  & p & LCC &  \\
\hline
HIP67260 &  &  & 7.03 & A0V &  &  & p & LCC &  \\
 &  &  & 8.37 &  & 0.44 & 228.9 & c &  &  \\
 &  &  & 14.70 &  & 2.22 & 77.1 & b &  &  \\
\hline
HIP67919 &  &  & 6.58 & A9V &  &  & p & LCC &  \\
 &  &  & 9.05 &  & 0.70 & 299.1 & nc &  &  \\
\hline
HIP68080 &  &  & 6.28 & A1V &  &  & p & UCL &  \\
 &  &  & 7.19 &  & 1.92 & 10.2 & c &  &  \\
\hline
HIP68532 &  &  & 7.03 & A3IV/V &  &  & p & UCL &  \\
 &  &  & 9.50 &  & 3.03 & 288.6 & nc &  &  \\
 &  &  & 10.53 &  & 3.15 & 291.7 & nc &  &  \\
\hline
HIP68781 &  &  & 7.38 & A2V &  &  & p & UCL &  \\
\hline
HIP68867 &  &  & 7.17 & A0V &  &  & p & UCL &  \\
 &  &  & 11.61 &  & 2.16 & 284.8 & nc &  &  \\
\hline
HIP68958 &  &  & 6.72 & Ap... &  &  & p & UCL &  \\
\hline
HIP69113 & 6.25 & 6.32 & 6.43 & B9V &  &  & p & UCL &  \\
 & 11.14 & 10.51 & 10.25 &  & 5.33 & 64.8 & nc &  &  \\
 & 11.19 & 10.46 & 10.23 &  & 5.52 & 66.9 & nc &  &  \\
\hline
HIP69749 &  &  & 6.62 & B9IV &  &  & p & UCL &  \\
 &  &  & 11.60 &  & 1.50 & 0.8 & nc &  &  \\
 &  &  & 12.69 &  & 8.10 & 50.0 & b &  &  \\
 &  &  & 13.40 &  & 5.57 & 352.4 & b &  &  \\
 &  &  & 14.16 &  & 8.79 & 62.5 & b &  &  \\
 &  &  & 14.48 &  & 9.13 & 66.8 & b &  &  \\
 &  &  & 14.51 &  & 4.43 & 278.6 & b &  &  \\
\hline
HIP69845 &  &  & 7.78 & B9V &  &  & p & UCL &  \\
\hline
HIP70441 &  &  & 7.31 & A1V &  &  & p & UCL &  \\
\hline
HIP70455 &  &  & 7.07 & B8V &  &  & p & UCL &  \\
\hline
HIP70626 &  &  & 6.56 & B9V &  &  & p & UCL &  \\
\hline
HIP70690 &  &  & 7.71 & B9V &  &  & p & UCL &  \\
\hline
HIP70697 &  &  & 7.17 & A0V &  &  & p & UCL &  \\
\hline
HIP70809 &  &  & 6.54 & Ap... &  &  & p & UCL &  \\
 &  &  & 14.64 &  & 4.97 & 214.4 & b &  &  \\
 &  &  & 14.60 &  & 8.72 & 297.3 & b &  &  \\
\hline
HIP70904 &  &  & 6.39 & A6V &  &  & p & UCL &  \\
 &  &  & 12.08 &  & 6.08 & 120.3 & b &  &  \\
 &  &  & 14.17 &  & 10.03 & 309.2 & b &  &  \\
\hline
HIP70918 &  &  & 6.35 & A0/A1V &  &  & p & UCL &  \\
\hline
HIP70998 &  &  & 7.06 & A1V &  &  & p & UCL &  \\
 &  &  & 10.83 &  & 1.17 & 354.6 & nc &  &  \\
\hline
HIP71140 &  &  & 7.13 & A7/A8IV &  &  & p & UCL &  \\
\hline
HIP71271 &  &  & 7.57 & A0V &  &  & p & UCL &  \\
\hline
HIP71321 &  &  & 7.17 & A9V &  &  & p & UCL &  \\
\hline
HIP71724 &  &  & 6.79 & B8/B9V &  &  & p & UCL &  \\
 &  &  & 9.70 &  & 8.66 & 23.0 & c &  &  \\
\hline
HIP71727 &  &  & 6.89 & A0p &  &  & p & UCL &  \\
 &  &  & 7.80 &  & 9.14 & 245.0 & c &  &  \\
\hline
HIP72140 &  &  & 7.09 & A1IV/V &  &  & p & UCL &  \\
 &  &  & 12.21 &  & 4.51 & 229.1 & b &  &  \\
\hline
HIP72192 & 6.71 & 6.71 & 6.71 & A0V &  &  & p & UCL &  \\
\hline
HIP72627 & 6.54 & 6.54 & 6.53 & A2V &  &  & p & UCL &  \\
\hline
HIP72940 &  &  & 6.85 & A1V &  &  & p & UCL &  \\
 &  &  & 8.57 &  & 3.16 & 221.6 & c &  &  \\
\hline
HIP72984 &  &  & 7.05 & A0/A1V &  &  & p & UCL &  \\
 &  &  & 14.37 &  & 5.83 & 118.1 & b &  &  \\
 &  &  & 8.50 &  & 4.71 & 260.3 & c &  &  \\
\hline
HIP73145 &  &  & 7.54 & A2IV &  &  & p & UCL &  \\
\hline
HIP73266 &  &  & 7.30 & B9V &  &  & p & UCL &  \\
\hline
HIP73341 &  &  & 6.67 & B8V &  &  & p & UCL &  \\
\hline
HIP73393 &  &  & 7.21 & A0V &  &  & p & UCL &  \\
\hline
HIP73937 &  &  & 6.05 & Ap &  &  & p & UCL &  \\
 &  &  & 14.05 &  & 3.48 & 30.5 & b &  &  \\
\hline
HIP74066 &  &  & 6.08 & B8IV &  &  & p & UCL &  \\
 &  &  & 8.43 &  & 1.22 & 109.6 & nc &  &  \\
\hline
HIP74100 &  &  & 6.12 & B7V &  &  & p & UCL &  \\
\hline
HIP74479 &  &  & 6.31 & B8V &  &  & p & UCL &  \\
 &  &  & 10.83 &  & 4.65 & 154.1 & nc &  &  \\
\hline
HIP74657 &  &  & 6.97 & B9IV &  &  & p & UCL &  \\
\hline
HIP74752 &  &  & 6.84 & B9V &  &  & p & UCL &  \\
 &  &  & 13.13 &  & 9.66 & 21.0 & b &  &  \\
\hline
HIP74797 &  &  & 7.55 & A2IV &  &  & p & UCL &  \\
\hline
HIP74985 &  &  & 7.53 & A0V &  &  & p & UCL &  \\
 &  &  & 13.13 &  & 6.37 & 145.2 & b &  &  \\
\hline
HIP75056 &  &  & 7.31 & A2V &  &  & p & UCL &  \\
 &  &  & 11.17 &  & 5.19 & 34.5 & nc &  &  \\
\hline
HIP75077 &  &  & 6.97 & A1V &  &  & p & UCL &  \\
\hline
HIP75151 &  &  & 6.65 & A+... &  &  & p & UCL &  \\
 &  &  & 8.09 &  & 5.70 & 120.9 & c &  &  \\
\hline
HIP75210 &  &  & 6.82 & B8/B9V &  &  & p & UCL &  \\
\hline
HIP75476 &  &  & 6.88 & A1/A2V &  &  & p & UCL &  \\
\hline
HIP75509 &  &  & 7.40 & A2V &  &  & p & UCL &  \\
\hline
HIP75647 &  &  & 5.86 & B5V &  &  & p & UCL &  \\
\hline
HIP75915 &  &  & 6.44 & B9V &  &  & p & UCL &  \\
 &  &  & 8.15 &  & 5.60 & 229.4 & c &  &  \\
\hline
HIP75957 &  &  & 7.24 & A0V &  &  & p & UCL &  \\
 &  &  & 13.41 &  & 5.56 & 105.7 & b &  &  \\
 &  &  & 13.21 &  & 9.21 & 227.1 & b &  &  \\
\hline
HIP76001 &  &  & 7.60 & A2/A3V &  &  & p & UCL &  \\
 &  &  & 7.80 &  & 0.25 & 3.2 & c &  &  \\
 &  &  & 8.20 &  & 1.48 & 124.8 & c &  &  \\
 &  &  & 12.85 &  & 6.58 & 127.5 & b &  &  \\
\hline
HIP76048 &  &  & 6.26 & B6/B7V &  &  & p & UCL &  \\
\hline
HIP76071 & 7.05 & 7.10 & 7.06 & B9V &  &  & p & US &  \\
 &  & 11.28 & 10.87 &  & 0.69 & 40.8 & nc &  &  \\
\hline
HIP76310 &  &  & 7.35 & A0V &  &  & p & US &  \\
\hline
HIP76503 &  &  & 6.25 & B9IV &  &  & p & US &  \\
\hline
HIP76633 &  &  & 7.51 & B9V &  &  & p & US &  \\
\hline
HIP77150 &  &  & 7.28 & A2V &  &  & p & UCL &  \\
\hline
HIP77295 &  &  & 7.64 & A2IV/V &  &  & p & UCL &  \\
 &  &  & 15.13 &  & 4.63 & 309.9 & b &  &  \\
%
\hline
HIP77315 &  &  & 7.24 & A0V   &       &       & p & UCL &  \\
 &  &  & 7.92 &  & 0.68 & 67.0 & c &  &  \\
HIP77317 &  &  & 7.37 & B9.5V & 37.37 & 137.3 & p & UCL &  \\
 &  &  & 14.24 &  & 32.78 & 146.8 & b &  &  \\
%HIP77317 &  &  & 7.37 & B9.5V &  &  & p & UCL &  \\
% &  &  & 14.24 &  & 7.37 & 270.3 & b &  &  \\
%
%
\hline
HIP77457 &  &  & 7.33 & A7IV &  &  & p & US &  \\
\hline
HIP77523 &  &  & 7.41 & B9V &  &  & p & UCL &  \\
\hline
HIP77858 &  &  & 5.40 & B5V &  &  & p & US &  \\
\hline
HIP77859 &  &  & 5.57 & B2V &  &  & p & US &  \\
\hline
HIP77900 &  &  & 6.44 & B7V &  &  & p & US &  \\
\hline
HIP77909 &  &  & 6.19 & B8III/IV &  &  & p & US &  \\
\hline
HIP77911 & 6.67 & 6.71 & 6.68 & B9V &  &  & p & US &  \\
 & 12.68 & 12.20 & 11.84 &  & 7.96 & 279.3 & nc &  &  \\
\hline
HIP77939 &  &  & 6.56 & B2/B3V &  &  & p & US &  \\
 &  &  & 8.09 &  & 0.52 & 119.1 & c &  &  \\
\hline
HIP77968 &  &  & 7.00 & B8V &  &  & p & UCL &  \\
 &  &  & 12.64 &  & 6.54 & 344.4 & b &  &  \\
 &  &  & 14.56 &  & 6.43 & 349.8 & b &  &  \\
\hline
HIP78099 &  &  & 7.35 & A0V &  &  & p & US &  \\
\hline
HIP78168 &  &  & 5.91 & B3V &  &  & p & US &  \\
\hline
HIP78196 &  &  & 7.08 & A0V &  &  & p & US &  \\
\hline
HIP78246 &  &  & 5.84 & B5V &  &  & p & US &  \\
\hline
HIP78494 &  &  & 7.11 & A2m... &  &  & p & US &  \\
\hline
HIP78530 & 6.87 & 6.92 & 6.87 & B9V &  &  & p & US &  \\
 &  & 14.56 & 14.22 &  & 4.54 & 139.7 & b &  &  \\
\hline
HIP78533 &  &  & 6.99 & Ap &  &  & p & UCL &  \\
 &  &  & 12.28 &  & 6.09 & 186.3 & b &  &  \\
\hline
HIP78541 &  &  & 6.99 & A0V &  &  & p & UCL &  \\
\hline
HIP78549 &  &  & 7.13 & B9.5V &  &  & p & US &  \\
 &  &  & 14.62 &  & 11.78 & 47.3 & b &  &  \\
\hline
HIP78663 &  &  & 7.76 & F5V &  &  & p & US &  \\
 &  &  & 13.42 &  & 8.88 & 103.0 & b &  &  \\
 &  &  & 15.41 &  & 6.11 & 184.7 & b &  &  \\
\hline
HIP78702 &  &  & 7.41 & B9V &  &  & p & US &  \\
\hline
HIP78754 &  &  & 6.95 & B8/B9V &  &  & p & UCL &  \\
\hline
HIP78756 &  &  & 7.16 & Ap &  &  & p & UCL &  \\
 &  &  & 9.52 &  & 8.63 & 216.4 & c &  &  \\
\hline
HIP78809 & 7.41 & 7.50 & 7.51 & B9V &  &  & p & US &  \\
 & 11.08 & 10.45 & 10.26 &  & 1.18 & 25.7 & nc &  &  \\
\hline
HIP78847 &  &  & 7.32 & A0V &  &  & p & US &  \\
 &  &  & 11.30 &  & 8.95 & 164.0 & nc &  &  \\
\hline
HIP78853 &  &  & 7.50 & A5V &  &  & p & UCL &  \\
 &  &  & 8.45 &  & 1.99 & 270.4 & c &  &  \\
 &  &  & 15.02 &  & 7.12 & 84.2 & b &  &  \\
\hline
HIP78877 &  &  & 6.08 & B8V &  &  & p & US &  \\
\hline
HIP78956 & 7.52 & 7.54 & 7.57 & B9.5V &  &  & p & US &  \\
 & 9.76 & 9.12 & 9.04 &  & 1.02 & 48.7 & nc &  &  \\
\hline
HIP78968 & 7.40 & 7.41 & 7.47 & B9V &  &  & p & US &  \\
 &  & 14.59 & 14.47 &  & 2.75 & 321.1 & b &  &  \\
\hline
HIP78996 &  &  & 7.46 & A9V &  &  & p & US &  \\
\hline
HIP79031 &  &  & 7.00 & B8IV/V &  &  & p & US &  \\
\hline
HIP79044 &  &  & 6.91 & B9V &  &  & p & UCL &  \\
 &  &  & 15.18 &  & 5.02 & 91.6 & b &  &  \\
\hline
HIP79098 &  &  & 5.90 & B9V &  &  & p & US &  \\
 &  &  & 14.10 &  & 2.37 & 116.8 & b &  &  \\
\hline
HIP79124 & 7.16 & 7.14 & 7.13 & A0V &  &  & p & US &  \\
 & 11.38 & 10.55 & 10.38 &  & 1.02 & 96.2 & nc &  &  \\
\hline
HIP79156 & 7.56 & 7.56 & 7.61 & A0V &  &  & p & US &  \\
 & 11.62 & 10.89 & 10.77 &  & 0.89 & 58.9 & nc &  &  \\
\hline
HIP79250 &  &  & 7.49 & A3III/IV &  &  & p & US &  \\
 &  &  & 10.71 &  & 0.62 & 180.9 & nc &  &  \\
\hline
HIP79366 &  &  & 7.47 & A3V &  &  & p & US &  \\
\hline
HIP79410 &  &  & 7.05 & B9V &  &  & p & US &  \\
 &  &  & 14.93 &  & 3.17 & 339.8 & b &  &  \\
%\hline
HIP79439 &  &  & 6.97 & B9V &  &  & p & US &  \\
\hline
HIP79530 &  &  & 6.60 & B6IV &  &  & p & US &  \\
 &  &  & 8.34 &  & 1.69 & 219.7 & c &  &  \\
\hline
HIP79599 &  &  & 6.30 & B9V &  &  & p & US &  \\
\hline
HIP79622 &  &  & 6.34 & B8V &  &  & p & US &  \\
\hline
HIP79631 &  &  & 7.17 & B9.5V &  &  & p & UCL &  \\
 &  &  & 7.61 &  & 2.94 & 127.9 & nc &  &  \\
 &  &  & 14.08 &  & 8.86 & 151.8 & b &  &  \\
\hline
HIP79739 &  &  & 7.24 & B8V &  &  & p & US &  \\
 &  &  & 11.60 &  & 0.94 & 118.6 & nc &  &  \\
\hline
HIP79771 &  &  & 7.09 & B9V &  &  & p & US &  \\
 &  &  & 10.94 &  & 3.66 & 313.6 & nc &  &  \\
\hline
HIP79785 &  &  & 6.41 & B9V &  &  & p & US &  \\
\hline
HIP79860 &  &  & 7.88 & A0V &  &  & p & US &  \\
\hline
HIP79878 &  &  & 7.06 & A0V &  &  & p & US &  \\
\hline
HIP79897 &  &  & 6.99 & B9V &  &  & p & US &  \\
\hline
HIP80019 &  &  & 7.08 & A0V &  &  & p & US &  \\
\hline
HIP80024 &  &  & 6.73 & B9II/III &  &  & p & US &  \\
\hline
HIP80059 &  &  & 7.44 & A7III/IV &  &  & p & US &  \\
\hline
HIP80126 &  &  & 6.44 & B6/B7Vn &  &  & p & US &  \\
\hline
HIP80142 &  &  & 6.60 & B7V &  &  & p & UCL &  \\
 &  &  & 12.16 &  & 8.54 & 44.0 & b &  &  \\
 &  &  & 9.53 &  & 9.32 & 216.2 & c &  &  \\
\hline
HIP80238 & 7.45 & 7.45 & 7.34 & A1III/IV &  &  & p & US &  \\
 & 7.96 & 7.66 & 7.49 &  & 1.03 & 318.5 & c &  &  \\
\hline
HIP80324 &  &  & 7.33 & A0V+... &  &  & p & US &  \\
 &  &  & 7.52 &  & 6.23 & 152.5 & c &  &  \\
\hline
HIP80371 &  &  & 6.40 & B5III &  &  & p & US &  \\
 &  &  & 8.92 &  & 2.73 & 140.6 & c &  &  \\
 &  &  & 13.36 &  & 9.22 & 32.0 & b &  &  \\
\hline
HIP80425 &  &  & 7.40 & A1V &  &  & p & US &  \\
 &  &  & 8.63 &  & 0.60 & 155.8 & c &  &  \\
\hline
HIP80461 &  &  & 5.92 & B3/B4V &  &  & p & US &  \\
 &  &  & 7.09 &  & 0.27 & 285.6 & c &  &  \\
\hline
HIP80474 & 6.13 & 6.08 & 5.76 & B5V &  &  & p & US & JH \\
 & 13.00 & 12.30 & 11.71 &  & 4.83 & 206.2 & nc &  & JH \\
\hline
HIP80493 &  &  & 7.05 & B9V &  &  & p & US &  \\
\hline
HIP80591 &  &  & 7.82 & A5V &  &  & p & UCL &  \\
\hline
HIP80799 & 7.68 & 7.75 & 7.46 & A2V &  &  & p & US & JH \\
 & 10.94 & 10.35 & 9.88 &  & 2.94 & 205.2 & nc &  & JH \\
\hline
HIP80896 &  &  & 7.53 & F3V &  &  & p & US &  \\
 &  &  & 10.51 &  & 2.28 & 177.0 & nc &  &  \\
\hline
HIP80897 &  &  & 7.78 & A0V &  &  & p & UCL &  \\
\hline
HIP81136 &  &  & 5.21 & A7/A8+... &  &  & p & UCL &  \\
\hline
HIP81316 &  &  & 6.72 & B9V &  &  & p & UCL &  \\
\hline
HIP81472 &  &  & 5.96 & B2.5IV &  &  & p & UCL &  \\
 &  &  & 13.23 &  & 5.21 & 357.5 & b &  &  \\
 &  &  & 13.20 &  & 4.52 & 274.4 & b &  &  \\
\hline
HIP81474 &  &  & 5.74 & B9.5IV &  &  & p & US &  \\
\hline
HIP81624 &  &  & 5.80 & A1V &  &  & p & US &  \\
 &  &  & 7.95 &  & 1.13 & 224.3 & c &  &  \\
\hline
HIP81751 &  &  & 8.29 & A9V &  &  & p & UCL &  \\
 &  &  & 12.18 &  & 8.91 & 68.0 & b &  &  \\
 &  &  & 14.44 &  & 6.12 & 219.6 & b &  &  \\
\hline
HIP81914 &  &  & 6.34 & B6/B7V &  &  & p & UCL &  \\
 &  &  & 12.29 &  & 6.18 & 49.5 & b &  &  \\
 &  &  & 14.28 &  & 9.11 & 39.8 & b &  &  \\
 &  &  & 14.61 &  & 5.15 & 286.2 & b &  &  \\
\hline
HIP81949 &  &  & 7.32 & A3V &  &  & p & UCL &  \\
 &  &  & 13.23 &  & 3.90 & 89.5 & b &  &  \\
 &  &  & 14.05 &  & 3.42 & 28.7 & b &  &  \\
 &  &  & 14.70 &  & 9.60 & 76.6 & b &  &  \\
 &  &  & 14.63 &  & 6.31 & 239.0 & b &  &  \\
 &  &  & 14.62 &  & 5.69 & 292.2 & b &  &  \\
 &  &  & 15.15 &  & 5.22 & 340.5 & b &  &  \\
 &  &  & 15.33 &  & 9.70 & 345.5 & b &  &  \\
\hline
HIP81972 &  &  & 5.92 & B3V &  &  & p & UCL &  \\
 &  &  & 10.57 &  & 2.01 & 312.0 & nc &  &  \\
 &  &  & 10.75 &  & 7.07 & 258.4 & c &  &  \\
 &  &  & 11.54 &  & 5.03 & 213.7 & nc &  &  \\
\hline
HIP82154 & 6.89 & 7.22 & 7.05 & B9IV/V &  &  & p & UCL & JH \\
 & 14.86 & 14.93 & 14.47 &  & 8.39 & 359.0 & b &  & JH \\
\hline
HIP82397 &  &  & 7.28 & A3V &  &  & p & US &  \\
 &  &  & 15.36 &  & 7.88 & 227.7 & b &  &  \\
\hline
HIP82430 &  &  & 7.25 & B9V &  &  & p & UCL &  \\
 &  &  & 12.41 &  & 4.59 & 96.1 & b &  &  \\
 &  &  & 14.03 &  & 5.98 & 65.3 & b &  &  \\
 &  &  & 14.29 &  & 6.08 & 329.3 & b &  &  \\
\hline
HIP82560 & 6.83 & 6.97 & 6.58 & A0V &  &  & p & UCL & JH \\
 &  & 13.86 & 12.76 &  & 4.73 & 4.6 & b &  & H \\
 &  & 14.40 & 13.13 &  & 3.94 & 222.0 & b &  & H \\
 &  & 14.38 & 13.68 &  & 6.20 & 283.3 & b &  & H \\
\hline
HIP83457 &  &  & 6.49 & A9V &  &  & p & UCL &  \\
\hline
HIP83542 &  &  & 5.38 & G8/K0III &  &  & p & US &  \\
 &  &  & 10.01 &  & 8.96 & 196.1 & nc &  &  \\
\hline
HIP83693 &  &  & 5.69 & A2IV &  &  & p & UCL &  \\
 &  &  & 9.26 &  & 5.82 & 78.4 & c &  &  \\
 &  &  & 13.64 &  & 12.69 & 134.9 & b &  &  \\


==> true_paper/ps/sos_largestrho.tex <==
HIP64004 & 25.1 & 7.92 & 0.68 & LCC & B1.5V \\ 
HIP71860 & 27.6 & 5.95 & 0.99 & UCL & B1.5III \\ 
HIP69113 & 28.6 & 4.57 & 1.34 & UCL & B9V \\ 
HIP75647 & 30.0 & 7.79 & 0.82 & UCL & B5V \\ 
HIP69749 & 30.2 & 4.07 & 1.59 & UCL & B9IV \\ 
HIP60320 & 32.4 & 9.71 & 0.71 & LCC & Am \\ 
HIP69618 & 33.9 & 6.71 & 1.08 & UCL & B4Vne \\ 
HIP77315 & 34.7 & 7.64 & 0.97 & UCL & A0V \\ 
HIP63003 & 34.8 & 8.64 & 0.86 & LCC & B2IV-V \\ 
HIP72192 & 35.3 & 7.72 & 0.98 & UCL & A0V \\ 
HIP69618 & 36.0 & 6.71 & 1.15 & UCL & B4Vne \\ 
HIP78104 & 38.3 & 7.97 & 1.03 & US & B2IV/V \\ 
HIP72984 & 39.0 & 5.93 & 1.41 & UCL & A0/A1V \\ 
HIP79374 & 41.4 & 7.47 & 1.19 & US & B2IV \\ 
HIP83693 & 43.3 & 7.73 & 1.20 & UCL & A2IV \\ 
HIP80024 & 46.7 & 6.98 & 1.43 & US & B9II/III \\ 
HIP67472 & 48.0 & 6.19 & 1.66 & UCL & B2IV/Ve \\ 
HIP78265 & 49.2 & 7.10 & 1.48 & US & B1V+B2V \\ 
HIP64661 & 60.0 & 8.04 & 1.60 & LCC & B8V \\ 
HIP65271 & 60.0 & 9.20 & 1.40 & LCC & B3V \\ 
HIP78384 & 115.0 & 6.61 & 3.73 & UCL & B2.5IV \\ 

